On Calibration and Out-of-domain Generalization

Out-of-domain (OOD) generalization is a significant challenge for machine learning models. Many techniques have been proposed to overcome this challenge, often focused on learning models with certain invariance properties. In this work, we draw a link between OOD performance and model calibration, arguing that calibration across multiple domains can be viewed as a special case of an invariant representation leading to better OOD generalization. Specifically, we show that under certain conditions, models which achieve \emph{multi-domain calibration} are provably free of spurious correlations. This leads us to propose multi-domain calibration as a measurable and trainable surrogate for the OOD performance of a classifier. We therefore introduce methods that are easy to apply and allow practitioners to improve multi-domain calibration by training or modifying an existing model, leading to better performance on unseen domains. Using four datasets from the recently proposed WILDS OOD benchmark, as well as the Colored MNIST dataset, we demonstrate that training or tuning models so they are calibrated across multiple domains leads to significantly improved performance on unseen test domains. We believe this intriguing connection between calibration and OOD generalization is promising from both a practical and theoretical point of view.

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations that we found most significant are discussed in \secref{sec:conc}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{The work does not treat a specific task where we see an immediate risk for negative societal impact. Though the methods described in this paper might be used by practitioners in safety-critical domains such as healthcare, and we suggest doing so with care since the suggested methods need to be studied further in controlled settings before being used in such domains.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{The paper conforms with the provided guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Most assumptions, such as population setting (infinite data) assumption, Gaussian data and linearity of models have been given in \secref{sec:motiv}. Other assumptions regarding specific general-position conditions under which the theorems hold are given in the supplementary material. along with detailed statements of the theorems.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{The proofs of main theoretical claims can be found in the supplementary material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We are preparing the code for publication and will do our best to have it ready by the end of the review period. Major parts of our code are based on existing publicly available code from papers that we cite, while noting that we used their published code. Hence some parts of our results can be reproduced quite easily by using it.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We specify hyperparameters and training details in the supplementary material (for both the WILDS benchmark and ColoredMNIST). When using a training setup from other works (e.g. in Colored MNIST), we give a reference to the work and specify changes we made upon their setup.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Some of the code we use is adapted from the works of \cite{arjovsky2019invariant, kamath2021does} which we cite several times and specifically in \secref{sec:exp} with regards to the used code. Our experiments on the WILDS benchmark \cite{koh2020wilds} use assets from the project that was also cited.}
  \item Did you mention the license of the assets?
    \answerYes{Licenses are included in the supplementary material.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All assets we use are allowed for public use for the purposes of sceintific research.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{The data we use is taken from publicly available datasets, where all personally identifiable information have been removed.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not conduct research with human subjects}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> distributionally_robust_calibration.tex <==
% \section{Calibration and Model Selection Methods}
% \section{Proactively Achieving Multi-Domain Calibration}
% \label{sec:method}

% Two valuable tools to assess calibration of a model are \emph{calibration plots} and scalar summaries such as the Expected Calibration Error, known as the \emph{ECE score}.\\
% \textbf{Calibration plots} \cite{degroot1983comparison} are a visual representation of model calibration in the case of binary labels. Each example $\x$ is placed into one of $B$ bins that partition the $[0,1]$ interval, in which the output, or \emph{confidence}, of the classifier $f(\x)$ falls. For each bin $b$, the accuracy of $f$ on the bin's examples $acc(b)$ is calculated along with the average confidence $conf(b)$. These are plotted against each other to form a curve, where deviations from a diagonal represent miscalibration.\\
% \textbf{ECE score} is one common scalar summary of the calibration curve, calculated by averaging the deviation between accuracy and confidence:
% \begin{equation} \label{eq:ece}
%     ECE = \sum^B_{b=1} \frac{n_b}{N} |acc(b) - conf(b)|.
% \end{equation}
% $n_b$ is the number of predictions in bin $b$, $N$ is the total number of data points.

To achieve the 
The main part of our experimental evaluation examines post-processing calibration techniques. We examine whether the extremely simple and computationally cheap act of calibrating a model can have an effect on OOD accuracy.
The other part examines the use of calibration scores for model selection.
As recently discussed by \cite{gulrajani2020search}, model selection is non-trivial when the goal is OOD generalization. They show that suboptimal model selection can eliminate the advantage that techniques designed for OOD generalization have over ERM with data augmentation.
As most model selection methods are based on accuracy, we consider a method based on the ECE score instead.

\subsection{Learning with Multi-Domain Calibration Error}


Binary classifiers are often calibrated using Platt Scaling \cite{platt1999probabilistic} or Isotonic Regression Scaling \cite{DBLP:conf/icml/ZadroznyE01, niculescu2005predicting}. For our experiments we compared these and several other techniques using the  ECE score they achieve \cite{naeini2015obtaining}. We wound up using Isotonic Regression as it usually outperformed the alternatives. The input to the method is a dataset $(f_i, y_i)_{i=1}^{N}$, where $f_i$ is a shorthand for the prediction of the model $f(\x)$ on the $i$-th datapoint and $y_i$ is the label. Isotonic Regression learns a \emph{monotonic} mapping $z:\reals\rightarrow\reals$ solving:
\begin{align*}
    (ISO)\quad\mathrm{arg}\min_{z}{\frac{1}{N}\sum_{i=1}^{N}{\left(z(f_i) - y_i\right)^2}}.
\end{align*}
Unlike standard calibration problems, we have multiple domains to calibrate over. In our experiments (\S \ref{sec:res}) we compare two methods for multi-domain calibration: naive calibration and distributionally robust calibration. 

\textbf{Naive Calibration} takes predictions of a trained model $f$ on validation data pooled from all domains and fits an isotonic regression $z^*$. We then report the performance of $z^* \circ f$ on the OOD test set.
\textbf{Robust Calibration.} In a multiple domain setting, Naive calibration may produce a model that is well calibrated on the pooled data, but uncalibrated on individual environments.
Motivated by the goal of simultaneous calibration, we offer the following alternative where we attempt to bound the worst-case misclaibration across environments. For each environment $e\in{E_{\text{train}}}$, we denote the number of validation examples we have from it by $N_{e}$, and by $f_{e,i}$ the prediction of the model on the $i$-th example. Then in a similar vein to robust optimization, robust isotonic regression solves:
\begin{align} \label{eq:robust_iso2}
    z^* = \mathrm{arg}\min_{z}\max_{e\in{E_{\text{train}}}}{\frac{1}{N_e}\sum_{i=1}^{N_e}{\left(z(f_{e,i})-y_i\right)^2}}.
\end{align}
Since Isotonic Regression can be cast as a Quadratic Program, and \eqref{eq:robust_iso2} minimizes a pointwise maximum on similar objectives, we can cast it as a convex program and solve with standard optimizers. In our implementation we use CVXPY \cite{diamond2016cvxpy}.
We then evaluate the OOD performance of $z^* \circ f$.

\subsection{Calibration Scores for Model Selection}
\begin{algorithm}
\caption{Model Selection with Worst-Case ECE}
\label{alg:model_selection}
\begin{algorithmic}[H]
\REQUIRE{Validation sets $\{(\mathbf{X}_i, \y_i)\}_{i=1}^{k}$, Models $\{f_j(\x)\}_{j=1}^{L}$}
\ENSURE{Selected model $f^*(\x)$}
\STATE Pool data from all environments to $(\mathbf{X},\mathbf{y})$
\STATE \textbf{for} $j\in{[L]}$ \textbf{do}
\begin{ALC@g}
\STATE $z_j \leftarrow ISO(f_j(\mathbf{X}), \y)$
    \STATE \textbf{for } $i\in{[k]}$ \textbf{do}
    \begin{ALC@g}
    \STATE $ECE_{i,j} \leftarrow ECE$ of $z_j\circ f_j$ on $(\mathbf{X}_i, \y_i)$
    \end{ALC@g}
    \end{ALC@g}
\STATE Return $f_j$ for $j\in{\mathrm{arg}\min_j\max_i{ECE_{i,j}}}$
\end{algorithmic}
\end{algorithm}
\vspace{-0.3cm}
The model selection procedure we examine takes $L$ pretrained models on $k$ training environments, along with validation sets for each environment. As described in \algref{alg:model_selection} it selects a model based on the best worst-case ECE over environments.
We follow \cite{naeini2015obtaining} and calibrate each model before calculating the ECE. This is important
since ECE can be very high on models that actually become well calibrated upon simple post-processing.
